SoccerNet-Caption: Dense Video Captioning for Soccer Broadcasts Commentaries

Soccer is more than just a game - it is a passion that transcends borders and unites people worldwide. From the roar of the crowds to the excitement of the commentators, every moment of a soccer match is a thrill. Yet, with so many games happening simultaneously, fans cannot watch them all live. Notifications for main actions can help, but lack the engagement of live commentary, leaving fans feeling disconnected. To fulfill this need, we propose in this paper a novel task of dense video captioning focusing on the generation of textual commentaries anchored with single timestamps. To support this task, we additionally present a challenging dataset consisting of almost 37k timestamped commentaries across 715.9 hours of soccer broadcast videos. Additionally, we propose a first benchmark and baseline for this task, highlighting the difficulty of temporally anchoring commentaries yet showing the capacity to generate meaningful commentaries. By providing broadcasters with a tool to summarize the content of their video with the same level of engagement as a live game, our method could help satisfy the needs of the numerous fans who follow their team but cannot necessarily watch the live game. We believe our method has the potential to enhance the accessibility and understanding of soccer content for a wider audience, bringing the excitement of the game to more people.

==> tables/results_spot_capt.tex <==

\begin{table}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l||c|c|c||c|c|c|c}
                        &               & \multicolumn{3}{c}{mAP@ (\%)}        \\ \cline{3-5}
        Encoder         & Aggregator    &      5 &     30 &     60 &   B@4  &    M  &     R  &      C \\ \midrule
        RN\_PCA         & NetVLAD       &    6.4 &   39.1 &   38.0 &   4.0 &   21.8 &   21.5 &   10.8 \\ %\hline
        RN\_PCA         & NetVLAD++     &    5.3 &   41.3 &   39.4 &   4.4 &   22.3 &   21.4 &   10.9 \\ %\hline
        RN\_PCA         & NetRVLAD      &    7.0 &   39.5 &   37.8 &   4.2 &   21.9 &   21.4 &   10.6 \\ %\hline
        RN\_PCA         & NetRVLAD++    &    5.4 &   41.5 &   39.4 &   4.2 &   21.8 &   21.2 &   11.0 \\ \midrule
        I3D\_PCA        & NetVLAD       &    4.5 &   33.0 &   33.3 &   3.2 &   21.9 &   20.4 &    7.5 \\ %\hline
        I3D\_PCA        & NetVLAD++     &    6.7 &   34.8 &   34.8 &   2.9 &   20.0 &   18.3 &    6.6 \\ %\hline
        I3D\_PCA        & NetRVLAD      &    4.1 &   32.8 &   32.3 &   3.1 &   21.1 &   20.7 &    8.0 \\ %\hline
        I3D\_PCA        & NetRVLAD++    &    5.9 &   34.5 &   34.1 &   3.7 &   21.7 &   20.8 &    9.2 \\ \midrule
        C3D\_PCA        & NetVLAD       &    4.8 &   38.1 &   37.1 &   3.9 &   21.9 &   21.4 &   10.3 \\ %\hline
        C3D\_PCA        & NetVLAD++     &    4.5 &   40.7 &   39.1 &   3.9 &   21.2 &   20.4 &   10.6 \\ %\hline
        C3D\_PCA        & NetRVLAD      &    6.9 &   39.3 &   38.1 &   4.0 &   21.6 &   21.1 &   11.0 \\ %\hline
        C3D\_PCA        & NetRVLAD++    &    3.9 &   39.2 &   38.2 &   3.9 &   21.3 &   20.7 &   11.0 \\ \midrule
        Baidu           & NetVLAD       &\bf10.5 &   42.1 &   40.7 &   5.7 &\bf23.6 &\bf23.5 &   15.7 \\ %\hline
        Baidu           & NetVLAD++     &    6.3 &\bf44.5 &\bf41.8 &   5.4 &   23.2 &   23.4 &\bf17.0 \\ %\hline
        Baidu           & NetRVLAD      &    6.7 &   39.5 &   38.7 &   5.5 &   23.5 &   23.2 &   15.4 \\ %\hline
        Baidu           & NetRVLAD++    &    3.6 &   44.0 &   41.2 &\bf5.7 &   23.5 &   23.3 &   16.0 \\
    \end{tabular}
    }
    \caption{
    \textbf{Spotting results.}
    We train our spotting model to detect and localize comments and compare different combinations of encoder and pooling modules.
    }
    \label{tab:spotting}
\end{table}

